The Orbit of WASP-12b is Decaying

WASP-12b is a transiting hot Jupiter on a 1.09-day orbit around a late-F star. Since the planet's discovery in 2008, the time interval between transits has been decreasing by $29\pm 2$ msec year$^{-1}$. This is a possible sign of orbital decay, although the previously available data left open the possibility that the planet's orbit is slightly eccentric and is undergoing apsidal precession. Here, we present new transit and occultation observations that provide more decisive evidence for orbital decay, which is favored over apsidal precession by a $\Delta\mathrm{BIC}$ of 22.3 or Bayes factor of 70,000. We also present new radial-velocity data that rule out the R{\o}mer effect as the cause of the period change. This makes WASP-12 the first planetary system for which we can be confident that the orbit is decaying. The decay timescale for the orbit is $P/\dot{P} = 3.25\pm 0.23$ Myr. Interpreting the decay as the result of tidal dissipation, the modified stellar tidal quality factor is $Q'_\star = 1.8 \times10^{5}$.

==> tables/.ipynb_checkpoints/timings-checkpoint.tex <==
% event, bjdtdb, err, epoch, source 
tra & 2454515.52496 & 0.00043 & -1640 & Hebb et al. (2009) \\
occ & 2454769.28190 & 0.00080 & -1408 & Campo et al. (2011) \\
occ & 2454773.64810 & 0.00060 & -1404 & Campo et al. (2011) \\
tra & 2454836.40340 & 0.00028 & -1346 & Copperwheat et al. (2013) \\
tra & 2454840.76893 & 0.00062 & -1342 & Chan et al. (2011) \\
tra & 2455140.90981 & 0.00042 & -1067 & Collins et al. (2017) \\
tra & 2455147.45861 & 0.00043 & -1061 & Maciejewski et al. (2013) \\
tra & 2455163.83061 & 0.00032 & -1046 & Collins et al. (2017) \\
tra & 2455172.56138 & 0.00036 & -1038 & Chan et al. (2011) \\
occ & 2455194.93440 & 0.00100 & -1018 & Croll et al. (2015) \\
occ & 2455202.57625 & 0.00220 & -1011 & Fohring et al. (2013) \\
tra & 2455209.66895 & 0.00046 & -1004 & Collins et al. (2017) \\
tra & 2455210.76151 & 0.00041 & -1003 & Collins et al. (2017) \\
tra & 2455230.40669 & 0.00019 & -985 & Maciejewski et al. (2013) \\
tra & 2455254.41871 & 0.00043 & -963 & Maciejewski et al. (2013) \\
tra & 2455494.52999 & 0.00072 & -743 & Maciejewski et al. (2013) \\
tra & 2455498.89590 & 0.00079 & -739 & Sada et al. (2012) \\
tra & 2455509.80971 & 0.00037 & -729 & Collins et al. (2017) \\
tra & 2455510.90218 & 0.00031 & -728 & Collins et al. (2017) \\
occ & 2455517.99514 & 0.00118 & -722 & Deming et al. (2015)^b \\
tra & 2455518.54070 & 0.00040 & -721 & Cowan et al. (2012) \\
tra & 2455542.55210 & 0.00040 & -699 & Cowan et al. (2012) \\
tra & 2455542.55273 & 0.00028 & -699 & Maciejewski et al. (2013) \\
tra & 2455566.56385 & 0.00028 & -677 & Maciejewski et al. (2013) \\
occ & 2455576.93200 & 0.00090 & -668 & Croll et al. (2015) \\
occ & 2455587.84730 & 0.00170 & -658 & Croll et al. (2015) \\
tra & 2455590.57561 & 0.00068 & -655 & Maciejewski et al. (2013) \\
tra & 2455598.21552 & 0.00035 & -648 & Maciejewski et al. (2013) \\
tra & 2455600.39800 & 0.00029 & -646 & Maciejewski et al. (2013) \\
tra & 2455601.49010 & 0.00024 & -645 & Maciejewski et al. (2013) \\
tra & 2455603.67261 & 0.00029 & -643 & Collins et al. (2017) \\
tra & 2455623.31829 & 0.00039 & -625 & Maciejewski et al. (2013) \\
tra & 2455876.52786 & 0.00027 & -393 & Maciejewski et al. (2013) \\
tra & 2455887.44198 & 0.00021 & -383 & Maciejewski et al. (2013) \\
tra & 2455888.53340 & 0.00027 & -382 & Maciejewski et al. (2013) \\
tra & 2455890.71635 & 0.00024 & -380 & Maciejewski et al. (2013) \\
tra & 2455903.81357 & 0.00032 & -368 & Collins et al. (2017) \\
occ & 2455910.90900 & 0.00130 & -362 & Crossfield et al. (2012) \\
tra & 2455920.18422 & 0.00031 & -353 & Maciejewski et al. (2013) \\
tra & 2455923.45850 & 0.00022 & -350 & Maciejewski et al. (2013) \\
occ & 2455924.00470 & 0.00210 & -350 & Croll et al. (2015) \\
tra & 2455946.37823 & 0.00018 & -329 & Maciejewski et al. (2013) \\
occ & 2455946.92290 & 0.00180 & -329 & Croll et al. (2015) \\
tra & 2455947.47015 & 0.00017 & -328 & Maciejewski et al. (2013) \\
tra & 2455948.56112 & 0.00033 & -327 & Maciejewski et al. (2013) \\
tra & 2455951.83534 & 0.00011 & -324 & Stevenson et al. (2014) \\
tra & 2455952.92720 & 0.00010 & -323 & Stevenson et al. (2014) \\
tra & 2455959.47543 & 0.00017 & -317 & Maciejewski et al. (2013) \\
tra & 2455960.56686 & 0.00032 & -316 & Maciejewski et al. (2013) \\
tra & 2455970.38941 & 0.00039 & -307 & Maciejewski et al. (2013) \\
tra & 2455971.48111 & 0.00035 & -306 & Maciejewski et al. (2013) \\
tra & 2455982.39509 & 0.00034 & -296 & Maciejewski et al. (2013) \\
tra & 2455983.48695 & 0.00035 & -295 & Maciejewski et al. (2013) \\
tra & 2455984.57797 & 0.00032 & -294 & Collins et al. (2017) \\
tra & 2455985.66975 & 0.00042 & -293 & Collins et al. (2017) \\
tra & 2455996.58378 & 0.00037 & -283 & Collins et al. (2017) \\
tra & 2456005.31533 & 0.00037 & -275 & Maciejewski et al. (2013) \\
tra & 2456006.40637 & 0.00031 & -274 & Maciejewski et al. (2013) \\
tra & 2456245.42729 & 0.00033 & -55 & Maciejewski et al. (2016) \\
tra & 2456249.79404 & 0.00039 & -51 & Collins et al. (2017) \\
tra & 2456273.80514 & 0.00030 & -29 & Collins et al. (2017) \\
tra & 2456282.53584 & 0.00030 & -21 & Maciejewski et al. (2016) \\
tra & 2456284.71857 & 0.00030 & -19 & Collins et al. (2017) \\
tra & 2456297.81605 & 0.00030 & -7 & Collins et al. (2017) \\
tra & 2456302.18179 & 0.00046 & -3 & Maciejewski et al. (2016) \\
tra & 2456305.45536 & 0.00024 & 0 & Maciejewski et al. (2016) \\
tra & 2456319.64424 & 0.00038 & 13 & Collins et al. (2017) \\
tra & 2456328.37556 & 0.00027 & 21 & Maciejewski et al. (2016) \\
tra & 2456329.46733 & 0.00029 & 22 & Maciejewski et al. (2016) \\
tra & 2456604.50489 & 0.00021 & 274 & Maciejewski et al. (2016) \\
tra & 2456605.59624 & 0.00030 & 275 & Maciejewski et al. (2016) \\
tra & 2456606.68760 & 0.00033 & 276 & Maciejewski et al. (2016) \\
tra & 2456607.77938 & 0.00071 & 277 & Collins et al. (2017) \\
tra & 2456629.60726 & 0.00019 & 297 & Maciejewski et al. (2016) \\
tra & 2456630.69917 & 0.00043 & 298 & Maciejewski et al. (2016) \\
occ & 2456638.88589 & 0.00110 & 305 & Patra et al. (2017) \\
occ & 2456642.15907 & 0.00141 & 308 & Patra et al. (2017) \\
tra & 2456654.71047 & 0.00034 & 320 & Collins et al. (2017) \\
tra & 2456659.07598 & 0.00034 & 324 & Kreidberg et al. (2015) \\
tra & 2456662.35014 & 0.00019 & 327 & Maciejewski et al. (2016) \\
tra & 2456663.44136 & 0.00019 & 328 & Maciejewski et al. (2016) \\
tra & 2456664.53256 & 0.00031 & 329 & Maciejewski et al. (2016) \\
tra & 2456674.35560 & 0.00028 & 338 & Kreidberg et al. (2015) \\
tra & 2456677.63039 & 0.00032 & 341 & Collins et al. (2017) \\
tra & 2456688.54384 & 0.00040 & 351 & Maciejewski et al. (2016) \\
tra & 2456694.00161 & 0.00029 & 356 & Kreidberg et al. (2015) \\
tra & 2456703.82417 & 0.00029 & 365 & Kreidberg et al. (2015) \\
tra & 2456711.46415 & 0.00025 & 372 & Maciejewski et al. (2016) \\
tra & 2456719.10428 & 0.00034 & 379 & Kreidberg et al. (2015) \\
tra & 2456721.28692 & 0.00034 & 381 & Kreidberg et al. (2015) \\
tra & 2456722.37807 & 0.00046 & 382 & Maciejewski et al. (2016) \\
tra & 2456986.50195 & 0.00043 & 624 & Maciejewski et al. (2016) \\
tra & 2457010.51298 & 0.00039 & 646 & Maciejewski et al. (2016) \\
tra & 2457012.69617 & 0.00049 & 648 & Collins et al. (2017) \\
tra & 2457045.43831 & 0.00046 & 678 & Maciejewski et al. (2016) \\
tra & 2457046.53019 & 0.00049 & 679 & Maciejewski et al. (2016) \\
tra & 2457059.62713 & 0.00035 & 691 & Collins et al. (2017) \\
tra & 2457060.71839 & 0.00036 & 692 & Collins et al. (2017) \\
tra & 2457067.26715 & 0.00022 & 698 & Maciejewski et al. (2016) \\
tra & 2457068.35834 & 0.00020 & 699 & Maciejewski et al. (2016) \\
tra & 2457103.28423 & 0.00031 & 731 & Maciejewski et al. (2016) \\
tra & 2457345.57867 & 0.00042 & 953 & Maciejewski et al. (2016) \\
tra & 2457390.32708 & 0.00033 & 994 & Maciejewski et al. (2016) \\
tra & 2457391.41818 & 0.00033 & 995 & Maciejewski et al. (2016) \\
tra & 2457426.34324 & 0.00055 & 1027 & Maciejewski et al. (2016) \\
tra & 2457427.43496 & 0.00023 & 1028 & Maciejewski et al. (2016) \\
tra & 2457451.44617 & 0.00021 & 1050 & Maciej+2019 \\
tra & 2457671.91324 & 0.00035 & 1252 & Patra et al. (2017) \\
tra & 2457691.55888 & 0.00025 & 1270 & Maciej+2019 \\
tra & 2457703.56388 & 0.00034 & 1281 & Maciej+2019 \\
tra & 2457706.83791 & 0.00037 & 1284 & Patra et al. (2017) \\
tra & 2457726.48400 & 0.00028 & 1302 & Maciej+2019 \\
tra & 2457727.57547 & 0.00023 & 1303 & Maciej+2019 \\
tra & 2457765.77515 & 0.00028 & 1338 & Patra et al. (2017) \\
tra & 2457766.86633 & 0.00039 & 1339 & Patra et al. (2017) \\
occ & 2457769.59573 & 0.00136 & 1341 & Hooton+2019 \\
tra & 2457772.32407 & 0.00024 & 1344 & Maciej+2019 \\
tra & 2457773.41517 & 0.00022 & 1345 & Maciej+2019 \\
tra & 2457776.68869 & 0.00029 & 1348 & Patra et al. (2017) \\
tra & 2457781.05418 & 0.00043 & 1352 & Patra et al. 2019 (in prep) \\
tra & 2457781.05566 & 0.00036 & 1352 & Patra et al. 2019 (in prep) \\
tra & 2457786.51210 & 0.00026 & 1357 & Maciej+2019 \\
tra & 2457788.69464 & 0.00048 & 1359 & Patra et al. (2017) \\
tra & 2457800.69978 & 0.00032 & 1370 & Patra et al. (2017) \\
tra & 2457808.34020 & 0.00040 & 1377 & Ozturk and Erdem (2019) \\
tra & 2457809.43190 & 0.00018 & 1378 & Maciej+2019 \\
tra & 2457810.52327 & 0.00021 & 1379 & Maciej+2019 \\
occ & 2457830.71389 & 0.00110 & 1397 & this work \\
tra & 2458026.62368 & 0.00056 & 1577 & Maciej+2019 \\
tra & 2458050.63519 & 0.00023 & 1599 & Maciej+2019 \\
tra & 2458060.45870 & 0.00030 & 1608 & Ozturk and Erdem (2019) \\
tra & 2458073.55509 & 0.00022 & 1620 & Maciej+2019 \\
tra & 2458074.64651 & 0.00034 & 1621 & Maciej+2019 \\
tra & 2458077.92107 & 0.00028 & 1624 & Patra et al. 2019 (in prep) \\
tra & 2458123.76011 & 0.00027 & 1666 & Patra et al. 2019 (in prep) \\
tra & 2458124.85183 & 0.00035 & 1667 & Patra et al. 2019 (in prep) \\
tra & 2458132.49121 & 0.00031 & 1674 & Maciej+2019 \\
tra & 2458134.67471 & 0.00032 & 1676 & Patra et al. 2019 (in prep) \\
tra & 2458136.85760 & 0.00033 & 1678 & Patra et al. 2019 (in prep) \\
tra & 2458155.41040 & 0.00050 & 1695 & Ozturk and Erdem (2019) \\
tra & 2458155.41152 & 0.00031 & 1695 & Maciej+2019 \\
tra & 2458156.50267 & 0.00032 & 1696 & Maciej+2019 \\
tra & 2458159.77773 & 0.00091 & 1699 & Patra et al. 2019 (in prep) \\
tra & 2458161.95991 & 0.00035 & 1701 & Patra et al. 2019 (in prep) \\
tra & 2458161.95964 & 0.00026 & 1701 & Patra et al. 2019 (in prep) \\
tra & 2458163.05125 & 0.00021 & 1702 & Patra et al. 2019 (in prep) \\
tra & 2458163.05089 & 0.00034 & 1702 & Patra et al. 2019 (in prep) \\
tra & 2458166.32575 & 0.00034 & 1705 & Maciej+2019 \\
tra & 2458178.33104 & 0.00038 & 1716 & Maciej+2019 \\
tra & 2458411.89495 & 0.00040 & 1930 & Patra et al. 2019 (in prep) \\
tra & 2458471.92257 & 0.00026 & 1985 & Patra et al. 2019 (in prep) \\
occ & 2458485.56424 & 0.00140 & 1997 & Von Essen+2019 \\
tra & 2458494.84270 & 0.00030 & 2006 & Patra et al. 2019 (in prep) \\
occ & 2458499.75572 & 0.00077 & 2010 & this work \\
occ & 2458504.11988 & 0.00087 & 2014 & this work \\
tra & 2458506.84758 & 0.00044 & 2017 & Patra et al. 2019 (in prep) \\
occ & 2458508.48459 & 0.00091 & 2018 & this work \\
occ & 2458517.21641 & 0.00074 & 2026 & this work \\


==> tables/hires_rvs.tex <==
% bjdtdb, mnvel, err_mnvel 
2455521.959432 & -136.635 & 2.534 \\
2455543.089922 & 5.728 & 2.919 \\
2455545.983884 & -162.390 & 2.822 \\
2455559.906718 & 141.616 & 2.345 \\
2455559.917563 & 115.818 & 2.727 \\
2455559.927852 & 111.001 & 3.186 \\
2455636.843302 & -143.932 & 2.627 \\
2455671.769904 & -107.997 & 2.446 \\
2455672.771896 & -195.600 & 2.524 \\
2455673.788031 & -205.391 & 2.790 \\
2455852.012615 & 68.746 & 3.147 \\
2455878.998057 & -215.632 & 3.830 \\
2455901.960764 & -196.872 & 2.933 \\
2455928.783714 & 149.753 & 2.613 \\
2455928.788760 & 147.510 & 2.588 \\
2455928.793864 & 147.804 & 2.606 \\
2455928.822776 & 115.802 & 2.226 \\
2455928.828771 & 113.554 & 2.163 \\
2455928.834859 & 103.195 & 2.273 \\
2455928.841109 & 92.281 & 2.205 \\
2455928.847232 & 96.068 & 2.036 \\
2455928.853297 & 74.408 & 2.035 \\
2455928.859153 & 74.816 & 2.355 \\
2455928.864987 & 63.350 & 2.383 \\
2455928.870739 & 75.198 & 2.376 \\
2455928.876584 & 63.670 & 2.220 \\
2455928.882313 & 51.474 & 2.208 \\
2455928.888146 & 43.809 & 2.156 \\
2455928.893841 & 43.629 & 2.247 \\
2455928.899639 & 23.763 & 2.250 \\
2455928.905658 & 24.191 & 2.127 \\
2455928.912232 & 18.021 & 2.312 \\
2455928.918563 & 5.739 & 2.196 \\
2455928.924488 & -8.812 & 2.295 \\
2455928.930425 & -15.142 & 2.068 \\
2455928.936120 & -17.130 & 2.177 \\
2455928.941710 & -39.543 & 2.173 \\
2455928.947393 & -29.895 & 2.137 \\
2455928.953064 & -38.645 & 2.427 \\
2455928.958712 & -50.172 & 2.118 \\
2455928.964349 & -55.586 & 2.070 \\
2455928.969881 & -55.857 & 2.304 \\
2455928.975564 & -59.190 & 2.052 \\
2455928.981155 & -62.572 & 2.224 \\
2455928.986814 & -66.610 & 2.119 \\
2455928.992567 & -70.651 & 2.334 \\
2455928.998574 & -81.305 & 2.182 \\
2455929.004916 & -92.700 & 2.230 \\
2455929.011178 & -92.870 & 2.402 \\
2455929.018099 & -110.688 & 2.326 \\
2455929.024870 & -109.396 & 2.366 \\
2456197.081787 & 207.626 & 3.515 \\
2456210.090854 & 172.022 & 3.111 \\
2456637.945245 & 204.835 & 3.161 \\
2457853.745487 & 164.479 & 2.941 \\
2457854.749059 & 26.408 & 2.898 \\
2458532.848410 & 212.650 & 2.978 \\
2455188.030545 & -167.966 & 3.451 \\
2455189.969831 & 70.320 & 2.665 \\
2455196.846861 & -197.549 & 2.726 \\
2455197.930084 & -212.529 & 4.296 \\
2455198.961510 & -187.556 & 2.927 \\
2455229.860339 & 25.135 & 3.324 \\
2455250.867142 & 227.277 & 2.675 \\
2455255.807886 & -212.759 & 2.218 \\
2455256.895765 & -210.776 & 2.599 \\
2455260.815214 & 174.936 & 2.615 \\
2455284.786727 & 210.274 & 2.941 \\
2455285.814022 & 230.239 & 4.003 \\
2455289.788595 & -102.288 & 2.347 \\
2455312.743830 & -58.250 & 2.780 \\
2455438.128228 & -174.900 & 2.824 \\


==> tables/timings.tex <==
% event, bjdtdb, err, epoch, source 
tra & 2454515.52496 & 0.00043 & -1640 & H09 \\
occ & 2454769.28190 & 0.00080 & -1408 & Ca11 \\
occ & 2454773.64810 & 0.00060 & -1404 & Ca11 \\
tra & 2454836.40340 & 0.00028 & -1346 & C13 \\
tra & 2454840.76893 & 0.00062 & -1342 & Ch11 \\
tra & 2455140.90981 & 0.00042 & -1067 & C17 \\
tra & 2455147.45861 & 0.00043 & -1061 & M13 \\
tra & 2455163.83061 & 0.00032 & -1046 & C17 \\
tra & 2455172.56138 & 0.00036 & -1038 & Ch11 \\
occ & 2455194.93440 & 0.00100 & -1018 & C15 \\
occ & 2455202.57625 & 0.00220 & -1011 & F13 \\
tra & 2455209.66895 & 0.00046 & -1004 & C17 \\
tra & 2455210.76151 & 0.00041 & -1003 & C17 \\
tra & 2455230.40669 & 0.00019 & -985 & M13 \\
tra & 2455254.41871 & 0.00043 & -963 & M13 \\
tra & 2455494.52999 & 0.00072 & -743 & M13 \\
tra & 2455498.89590 & 0.00079 & -739 & S12 \\
tra & 2455509.80971 & 0.00037 & -729 & C17 \\
tra & 2455510.90218 & 0.00031 & -728 & C17 \\
occ & 2455517.99514 & 0.00118 & -722 & D15 \\
tra & 2455518.54070 & 0.00040 & -721 & Co12 \\
tra & 2455542.55210 & 0.00040 & -699 & Co12 \\
tra & 2455542.55273 & 0.00028 & -699 & M13 \\
tra & 2455566.56385 & 0.00028 & -677 & M13 \\
occ & 2455576.93200 & 0.00090 & -668 & C15 \\
occ & 2455587.84730 & 0.00170 & -658 & C15 \\
tra & 2455590.57561 & 0.00068 & -655 & M13 \\
tra & 2455598.21552 & 0.00035 & -648 & M13 \\
tra & 2455600.39800 & 0.00029 & -646 & M13 \\
tra & 2455601.49010 & 0.00024 & -645 & M13 \\
tra & 2455603.67261 & 0.00029 & -643 & C17 \\
tra & 2455623.31829 & 0.00039 & -625 & M13 \\
tra & 2455876.52786 & 0.00027 & -393 & M13 \\
tra & 2455887.44198 & 0.00021 & -383 & M13 \\
tra & 2455888.53340 & 0.00027 & -382 & M13 \\
tra & 2455890.71635 & 0.00024 & -380 & M13 \\
tra & 2455903.81357 & 0.00032 & -368 & C17 \\
occ & 2455910.90900 & 0.00130 & -362 & Cr12 \\
tra & 2455920.18422 & 0.00031 & -353 & M13 \\
tra & 2455923.45850 & 0.00022 & -350 & M13 \\
occ & 2455924.00470 & 0.00210 & -350 & C15 \\
tra & 2455946.37823 & 0.00018 & -329 & M13 \\
occ & 2455946.92290 & 0.00180 & -329 & C15 \\
tra & 2455947.47015 & 0.00017 & -328 & M13 \\
tra & 2455948.56112 & 0.00033 & -327 & M13 \\
tra & 2455951.83534 & 0.00011 & -324 & S14 \\
tra & 2455952.92720 & 0.00010 & -323 & S14 \\
tra & 2455959.47543 & 0.00017 & -317 & M13 \\
tra & 2455960.56686 & 0.00032 & -316 & M13 \\
tra & 2455970.38941 & 0.00039 & -307 & M13 \\
tra & 2455971.48111 & 0.00035 & -306 & M13 \\
tra & 2455982.39509 & 0.00034 & -296 & M13 \\
tra & 2455983.48695 & 0.00035 & -295 & M13 \\
tra & 2455984.57797 & 0.00032 & -294 & C17 \\
tra & 2455985.66975 & 0.00042 & -293 & C17 \\
tra & 2455996.58378 & 0.00037 & -283 & C17 \\
tra & 2456005.31533 & 0.00037 & -275 & M13 \\
tra & 2456006.40637 & 0.00031 & -274 & M13 \\
tra & 2456245.42729 & 0.00033 & -55 & M16 \\
tra & 2456249.79404 & 0.00039 & -51 & C17 \\
tra & 2456273.80514 & 0.00030 & -29 & C17 \\
tra & 2456282.53584 & 0.00030 & -21 & M16 \\
tra & 2456284.71857 & 0.00030 & -19 & C17 \\
tra & 2456297.81605 & 0.00030 & -7 & C17 \\
tra & 2456302.18179 & 0.00046 & -3 & M16 \\
tra & 2456305.45536 & 0.00024 & 0 & M16 \\
tra & 2456319.64424 & 0.00038 & 13 & C17 \\
tra & 2456328.37556 & 0.00027 & 21 & M16 \\
tra & 2456329.46733 & 0.00029 & 22 & M16 \\
tra & 2456604.50489 & 0.00021 & 274 & M16 \\
tra & 2456605.59624 & 0.00030 & 275 & M16 \\
tra & 2456606.68760 & 0.00033 & 276 & M16 \\
tra & 2456607.77938 & 0.00071 & 277 & C17 \\
tra & 2456629.60726 & 0.00019 & 297 & M16 \\
tra & 2456630.69917 & 0.00043 & 298 & M16 \\
occ & 2456638.88589 & 0.00110 & 305 & P17 \\
occ & 2456642.15907 & 0.00141 & 308 & P17 \\
tra & 2456654.71047 & 0.00034 & 320 & C17 \\
tra & 2456659.07598 & 0.00034 & 324 & K15 \\
tra & 2456662.35014 & 0.00019 & 327 & M16 \\
tra & 2456663.44136 & 0.00019 & 328 & M16 \\
tra & 2456664.53256 & 0.00031 & 329 & M16 \\
tra & 2456674.35560 & 0.00028 & 338 & K15 \\
tra & 2456677.63039 & 0.00032 & 341 & C17 \\
tra & 2456688.54384 & 0.00040 & 351 & M16 \\
tra & 2456694.00161 & 0.00029 & 356 & K15 \\
tra & 2456703.82417 & 0.00029 & 365 & K15 \\
tra & 2456711.46415 & 0.00025 & 372 & M16 \\
tra & 2456719.10428 & 0.00034 & 379 & K15 \\
tra & 2456721.28692 & 0.00034 & 381 & K15 \\
tra & 2456722.37807 & 0.00046 & 382 & M16 \\
tra & 2456986.50195 & 0.00043 & 624 & M16 \\
tra & 2457010.51298 & 0.00039 & 646 & M16 \\
tra & 2457012.69617 & 0.00049 & 648 & C17 \\
tra & 2457045.43831 & 0.00046 & 678 & M16 \\
tra & 2457046.53019 & 0.00049 & 679 & M16 \\
tra & 2457059.62713 & 0.00035 & 691 & C17 \\
tra & 2457060.71839 & 0.00036 & 692 & C17 \\
tra & 2457067.26715 & 0.00022 & 698 & M16 \\
tra & 2457068.35834 & 0.00020 & 699 & M16 \\
tra & 2457103.28423 & 0.00031 & 731 & M16 \\
tra & 2457345.57867 & 0.00042 & 953 & M16 \\
tra & 2457390.32708 & 0.00033 & 994 & M16 \\
tra & 2457391.41818 & 0.00033 & 995 & M16 \\
tra & 2457426.34324 & 0.00055 & 1027 & M16 \\
tra & 2457427.43496 & 0.00023 & 1028 & M16 \\
tra & 2457451.44617 & 0.00021 & 1050 & M18 \\
tra & 2457671.91324 & 0.00035 & 1252 & P17 \\
tra & 2457691.55888 & 0.00025 & 1270 & M18 \\
tra & 2457703.56388 & 0.00034 & 1281 & M18 \\
tra & 2457706.83791 & 0.00037 & 1284 & P17 \\
tra & 2457726.48400 & 0.00028 & 1302 & M18 \\
tra & 2457727.57547 & 0.00023 & 1303 & M18 \\
tra & 2457765.77515 & 0.00028 & 1338 & P17 \\
tra & 2457766.86633 & 0.00039 & 1339 & P17 \\
occ & 2457769.59573 & 0.00136 & 1341 & H19 \\
tra & 2457772.32407 & 0.00024 & 1344 & M18 \\
tra & 2457773.41517 & 0.00022 & 1345 & M18 \\
tra & 2457776.68869 & 0.00029 & 1348 & P17 \\
tra & 2457781.05418 & 0.00043 & 1352 & P19 \\
tra & 2457781.05566 & 0.00036 & 1352 & P19 \\
tra & 2457786.51210 & 0.00026 & 1357 & M18 \\
tra & 2457788.69464 & 0.00048 & 1359 & P17 \\
tra & 2457800.69978 & 0.00032 & 1370 & P17 \\
tra & 2457808.34020 & 0.00040 & 1377 & O19 \\
tra & 2457809.43190 & 0.00018 & 1378 & M18 \\
tra & 2457810.52327 & 0.00021 & 1379 & M18 \\
occ & 2457830.71389 & 0.00110 & 1397 & this work \\
tra & 2458026.62368 & 0.00056 & 1577 & M18 \\
tra & 2458050.63519 & 0.00023 & 1599 & M18 \\
tra & 2458060.45870 & 0.00030 & 1608 & O19 \\
tra & 2458073.55509 & 0.00022 & 1620 & M18 \\
tra & 2458074.64651 & 0.00034 & 1621 & M18 \\
tra & 2458077.92107 & 0.00028 & 1624 & this work \\
tra & 2458123.76011 & 0.00027 & 1666 & this work \\
tra & 2458124.85183 & 0.00035 & 1667 & this work \\
tra & 2458132.49121 & 0.00031 & 1674 & M18 \\
tra & 2458134.67471 & 0.00032 & 1676 & this work \\
tra & 2458136.85760 & 0.00033 & 1678 & this work \\
tra & 2458155.41040 & 0.00050 & 1695 & O19 \\
tra & 2458155.41152 & 0.00031 & 1695 & M18 \\
tra & 2458156.50267 & 0.00032 & 1696 & M18 \\
tra & 2458159.77773 & 0.00091 & 1699 & this work \\
tra & 2458161.95991 & 0.00035 & 1701 & P19 \\
tra & 2458161.95964 & 0.00026 & 1701 & P19 \\
tra & 2458163.05125 & 0.00021 & 1702 & P19 \\
tra & 2458163.05089 & 0.00034 & 1702 & P19 \\
tra & 2458166.32575 & 0.00034 & 1705 & M18 \\
tra & 2458178.33104 & 0.00038 & 1716 & M18 \\
tra & 2458411.89495 & 0.00040 & 1930 & this work \\
tra & 2458471.92257 & 0.00026 & 1985 & this work \\
occ & 2458485.56424 & 0.00140 & 1997 & V19 \\
tra & 2458494.84270 & 0.00030 & 2006 & this work \\
occ & 2458499.75572 & 0.00077 & 2010 & this work \\
occ & 2458504.11988 & 0.00087 & 2014 & this work \\
tra & 2458506.84758 & 0.00044 & 2017 & this work \\
occ & 2458508.48459 & 0.00091 & 2018 & this work \\
occ & 2458517.21641 & 0.00074 & 2026 & this work \\


==> tables/timings_fullsource.tex <==
tra & 2454515.52496 & 0.00043 & -1640 & Hebb et al. (2009) \\
occ & 2454769.28190 & 0.00080 & -1408 & Campo et al. (2011) \\
occ & 2454773.64810 & 0.00060 & -1404 & Campo et al. (2011) \\
tra & 2454836.40340 & 0.00028 & -1346 & Copperwheat et al. (2013) \\
tra & 2454840.76893 & 0.00062 & -1342 & Chan et al. (2011) \\
tra & 2455140.90981 & 0.00042 & -1067 & Collins et al. (2017) \\
tra & 2455147.45861 & 0.00043 & -1061 & Maciejewski et al. (2013) \\
tra & 2455163.83061 & 0.00032 & -1046 & Collins et al. (2017) \\
tra & 2455172.56138 & 0.00036 & -1038 & Chan et al. (2011) \\
occ & 2455194.93440 & 0.00100 & -1018 & Croll et al. (2015) \\
occ & 2455202.57625 & 0.00220 & -1011 & Fohring et al. (2013) \\
tra & 2455209.66895 & 0.00046 & -1004 & Collins et al. (2017) \\
tra & 2455210.76151 & 0.00041 & -1003 & Collins et al. (2017) \\
tra & 2455230.40669 & 0.00019 & -985 & Maciejewski et al. (2013) \\
tra & 2455254.41871 & 0.00043 & -963 & Maciejewski et al. (2013) \\
tra & 2455494.52999 & 0.00072 & -743 & Maciejewski et al. (2013) \\
tra & 2455498.89590 & 0.00079 & -739 & Sada et al. (2012) \\
tra & 2455509.80971 & 0.00037 & -729 & Collins et al. (2017) \\
tra & 2455510.90218 & 0.00031 & -728 & Collins et al. (2017) \\
occ & 2455517.99514 & 0.00118 & -722 & Deming et al. (2015) \\
tra & 2455518.54070 & 0.00040 & -721 & Cowan et al. (2012) \\
tra & 2455542.55210 & 0.00040 & -699 & Cowan et al. (2012) \\
tra & 2455542.55273 & 0.00028 & -699 & Maciejewski et al. (2013) \\
tra & 2455566.56385 & 0.00028 & -677 & Maciejewski et al. (2013) \\
occ & 2455576.93200 & 0.00090 & -668 & Croll et al. (2015) \\
occ & 2455587.84730 & 0.00170 & -658 & Croll et al. (2015) \\
tra & 2455590.57561 & 0.00068 & -655 & Maciejewski et al. (2013) \\
tra & 2455598.21552 & 0.00035 & -648 & Maciejewski et al. (2013) \\
tra & 2455600.39800 & 0.00029 & -646 & Maciejewski et al. (2013) \\
tra & 2455601.49010 & 0.00024 & -645 & Maciejewski et al. (2013) \\
tra & 2455603.67261 & 0.00029 & -643 & Collins et al. (2017) \\
tra & 2455623.31829 & 0.00039 & -625 & Maciejewski et al. (2013) \\
tra & 2455876.52786 & 0.00027 & -393 & Maciejewski et al. (2013) \\
tra & 2455887.44198 & 0.00021 & -383 & Maciejewski et al. (2013) \\
tra & 2455888.53340 & 0.00027 & -382 & Maciejewski et al. (2013) \\
tra & 2455890.71635 & 0.00024 & -380 & Maciejewski et al. (2013) \\
tra & 2455903.81357 & 0.00032 & -368 & Collins et al. (2017) \\
occ & 2455910.90900 & 0.00130 & -362 & Crossfield et al. (2012) \\
tra & 2455920.18422 & 0.00031 & -353 & Maciejewski et al. (2013) \\
tra & 2455923.45850 & 0.00022 & -350 & Maciejewski et al. (2013) \\
occ & 2455924.00470 & 0.00210 & -350 & Croll et al. (2015) \\
tra & 2455946.37823 & 0.00018 & -329 & Maciejewski et al. (2013) \\
occ & 2455946.92290 & 0.00180 & -329 & Croll et al. (2015) \\
tra & 2455947.47015 & 0.00017 & -328 & Maciejewski et al. (2013) \\
tra & 2455948.56112 & 0.00033 & -327 & Maciejewski et al. (2013) \\
tra & 2455951.83534 & 0.00011 & -324 & Stevenson et al. (2014) \\
tra & 2455952.92720 & 0.00010 & -323 & Stevenson et al. (2014) \\
tra & 2455959.47543 & 0.00017 & -317 & Maciejewski et al. (2013) \\
tra & 2455960.56686 & 0.00032 & -316 & Maciejewski et al. (2013) \\
tra & 2455970.38941 & 0.00039 & -307 & Maciejewski et al. (2013) \\
tra & 2455971.48111 & 0.00035 & -306 & Maciejewski et al. (2013) \\
tra & 2455982.39509 & 0.00034 & -296 & Maciejewski et al. (2013) \\
tra & 2455983.48695 & 0.00035 & -295 & Maciejewski et al. (2013) \\
tra & 2455984.57797 & 0.00032 & -294 & Collins et al. (2017) \\
tra & 2455985.66975 & 0.00042 & -293 & Collins et al. (2017) \\
tra & 2455996.58378 & 0.00037 & -283 & Collins et al. (2017) \\
tra & 2456005.31533 & 0.00037 & -275 & Maciejewski et al. (2013) \\
tra & 2456006.40637 & 0.00031 & -274 & Maciejewski et al. (2013) \\
tra & 2456245.42729 & 0.00033 & -55 & Maciejewski et al. (2016) \\
tra & 2456249.79404 & 0.00039 & -51 & Collins et al. (2017) \\
tra & 2456273.80514 & 0.00030 & -29 & Collins et al. (2017) \\
tra & 2456282.53584 & 0.00030 & -21 & Maciejewski et al. (2016) \\
tra & 2456284.71857 & 0.00030 & -19 & Collins et al. (2017) \\
tra & 2456297.81605 & 0.00030 & -7 & Collins et al. (2017) \\
tra & 2456302.18179 & 0.00046 & -3 & Maciejewski et al. (2016) \\
tra & 2456305.45536 & 0.00024 & 0 & Maciejewski et al. (2016) \\
tra & 2456319.64424 & 0.00038 & 13 & Collins et al. (2017) \\
tra & 2456328.37556 & 0.00027 & 21 & Maciejewski et al. (2016) \\
tra & 2456329.46733 & 0.00029 & 22 & Maciejewski et al. (2016) \\
tra & 2456604.50489 & 0.00021 & 274 & Maciejewski et al. (2016) \\
tra & 2456605.59624 & 0.00030 & 275 & Maciejewski et al. (2016) \\
tra & 2456606.68760 & 0.00033 & 276 & Maciejewski et al. (2016) \\
tra & 2456607.77938 & 0.00071 & 277 & Collins et al. (2017) \\
tra & 2456629.60726 & 0.00019 & 297 & Maciejewski et al. (2016) \\
tra & 2456630.69917 & 0.00043 & 298 & Maciejewski et al. (2016) \\
occ & 2456638.88589 & 0.00110 & 305 & Patra et al. (2017) \\
occ & 2456642.15907 & 0.00141 & 308 & Patra et al. (2017) \\
tra & 2456654.71047 & 0.00034 & 320 & Collins et al. (2017) \\
tra & 2456659.07598 & 0.00034 & 324 & Kreidberg et al. (2015) \\
tra & 2456662.35014 & 0.00019 & 327 & Maciejewski et al. (2016) \\
tra & 2456663.44136 & 0.00019 & 328 & Maciejewski et al. (2016) \\
tra & 2456664.53256 & 0.00031 & 329 & Maciejewski et al. (2016) \\
tra & 2456674.35560 & 0.00028 & 338 & Kreidberg et al. (2015) \\
tra & 2456677.63039 & 0.00032 & 341 & Collins et al. (2017) \\
tra & 2456688.54384 & 0.00040 & 351 & Maciejewski et al. (2016) \\
tra & 2456694.00161 & 0.00029 & 356 & Kreidberg et al. (2015) \\
tra & 2456703.82417 & 0.00029 & 365 & Kreidberg et al. (2015) \\
tra & 2456711.46415 & 0.00025 & 372 & Maciejewski et al. (2016) \\
tra & 2456719.10428 & 0.00034 & 379 & Kreidberg et al. (2015) \\
tra & 2456721.28692 & 0.00034 & 381 & Kreidberg et al. (2015) \\
tra & 2456722.37807 & 0.00046 & 382 & Maciejewski et al. (2016) \\
tra & 2456986.50195 & 0.00043 & 624 & Maciejewski et al. (2016) \\
tra & 2457010.51298 & 0.00039 & 646 & Maciejewski et al. (2016) \\
tra & 2457012.69617 & 0.00049 & 648 & Collins et al. (2017) \\
tra & 2457045.43831 & 0.00046 & 678 & Maciejewski et al. (2016) \\
tra & 2457046.53019 & 0.00049 & 679 & Maciejewski et al. (2016) \\
tra & 2457059.62713 & 0.00035 & 691 & Collins et al. (2017) \\
tra & 2457060.71839 & 0.00036 & 692 & Collins et al. (2017) \\
tra & 2457067.26715 & 0.00022 & 698 & Maciejewski et al. (2016) \\
tra & 2457068.35834 & 0.00020 & 699 & Maciejewski et al. (2016) \\
tra & 2457103.28423 & 0.00031 & 731 & Maciejewski et al. (2016) \\
tra & 2457345.57867 & 0.00042 & 953 & Maciejewski et al. (2016) \\
tra & 2457390.32708 & 0.00033 & 994 & Maciejewski et al. (2016) \\
tra & 2457391.41818 & 0.00033 & 995 & Maciejewski et al. (2016) \\
tra & 2457426.34324 & 0.00055 & 1027 & Maciejewski et al. (2016) \\
tra & 2457427.43496 & 0.00023 & 1028 & Maciejewski et al. (2016) \\
tra & 2457451.44617 & 0.00021 & 1050 & Maciejewski et al. (2018) \\
tra & 2457671.91324 & 0.00035 & 1252 & Patra et al. (2017) \\
tra & 2457691.55888 & 0.00025 & 1270 & Maciejewski et al. (2018) \\
tra & 2457703.56388 & 0.00034 & 1281 & Maciejewski et al. (2018) \\
tra & 2457706.83791 & 0.00037 & 1284 & Patra et al. (2017) \\
tra & 2457726.48400 & 0.00028 & 1302 & Maciejewski et al. (2018) \\
tra & 2457727.57547 & 0.00023 & 1303 & Maciejewski et al. (2018) \\
tra & 2457765.77515 & 0.00028 & 1338 & Patra et al. (2017) \\
tra & 2457766.86633 & 0.00039 & 1339 & Patra et al. (2017) \\
occ & 2457769.59573 & 0.00136 & 1341 & Hooton et al. (2019) \\
tra & 2457772.32407 & 0.00024 & 1344 & Maciejewski et al. (2018) \\
tra & 2457773.41517 & 0.00022 & 1345 & Maciejewski et al. (2018) \\
tra & 2457776.68869 & 0.00029 & 1348 & Patra et al. (2017) \\
tra & 2457781.05418 & 0.00043 & 1352 & Patra et al. 2019 (in prep) \\
tra & 2457781.05566 & 0.00036 & 1352 & Patra et al. 2019 (in prep) \\
tra & 2457786.51210 & 0.00026 & 1357 & Maciejewski et al. (2018) \\
tra & 2457788.69464 & 0.00048 & 1359 & Patra et al. (2017) \\
tra & 2457800.69978 & 0.00032 & 1370 & Patra et al. (2017) \\
tra & 2457808.34020 & 0.00040 & 1377 & Ozturk and Erdem (2019) \\
tra & 2457809.43190 & 0.00018 & 1378 & Maciejewski et al. (2018) \\
tra & 2457810.52327 & 0.00021 & 1379 & Maciejewski et al. (2018) \\
occ & 2457830.71389 & 0.00110 & 1397 & this work \\
tra & 2458026.62368 & 0.00056 & 1577 & Maciejewski et al. (2018) \\
tra & 2458050.63519 & 0.00023 & 1599 & Maciejewski et al. (2018) \\
tra & 2458060.45870 & 0.00030 & 1608 & Ozturk and Erdem (2019) \\
tra & 2458073.55509 & 0.00022 & 1620 & Maciejewski et al. (2018) \\
tra & 2458074.64651 & 0.00034 & 1621 & Maciejewski et al. (2018) \\
tra & 2458077.92107 & 0.00028 & 1624 & this work \\
tra & 2458123.76011 & 0.00027 & 1666 & this work \\
tra & 2458124.85183 & 0.00035 & 1667 & this work \\
tra & 2458132.49121 & 0.00031 & 1674 & Maciejewski et al. (2018) \\
tra & 2458134.67471 & 0.00032 & 1676 & this work \\
tra & 2458136.85760 & 0.00033 & 1678 & this work \\
tra & 2458155.41040 & 0.00050 & 1695 & Ozturk and Erdem (2019) \\
tra & 2458155.41152 & 0.00031 & 1695 & Maciejewski et al. (2018) \\
tra & 2458156.50267 & 0.00032 & 1696 & Maciejewski et al. (2018) \\
tra & 2458159.77773 & 0.00091 & 1699 & this work \\
tra & 2458161.95991 & 0.00035 & 1701 & Patra et al. 2019 (in prep) \\
tra & 2458161.95964 & 0.00026 & 1701 & Patra et al. 2019 (in prep) \\
tra & 2458163.05125 & 0.00021 & 1702 & Patra et al. 2019 (in prep) \\
tra & 2458163.05089 & 0.00034 & 1702 & Patra et al. 2019 (in prep) \\
tra & 2458166.32575 & 0.00034 & 1705 & Maciejewski et al. (2018) \\
tra & 2458178.33104 & 0.00038 & 1716 & Maciejewski et al. (2018) \\
tra & 2458411.89495 & 0.00040 & 1930 & this work \\
tra & 2458471.92257 & 0.00026 & 1985 & this work \\
occ & 2458485.56424 & 0.00140 & 1997 & Von Essen et al. (2019) \\
tra & 2458494.84270 & 0.00030 & 2006 & this work \\
occ & 2458499.75572 & 0.00077 & 2010 & this work \\
occ & 2458504.11988 & 0.00087 & 2014 & this work \\
tra & 2458506.84758 & 0.00044 & 2017 & this work \\
occ & 2458508.48459 & 0.00091 & 2018 & this work \\
occ & 2458517.21641 & 0.00074 & 2026 & this work \\

